A Continuous-Time Stochastic Process for High-Resolution Network Data in Sports

Technological advances have paved the way for collecting high-resolution network data in basketball, football, and other team-based sports. Such data consist of interactions among players of competing teams indexed by space and time. High-resolution network data are vital to understanding and predicting the performance of teams, because the performance of a team is more than the sum of the strengths of its individual players: Whether a collection of players forms a strong team depends on the strength of the individual players as well as the interactions among the players. We introduce a continuous-time stochastic process as a model of interactions among players of competing teams indexed by space and time, discuss basic properties of the continuous-time stochastic process, and learn the stochastic process from high-resolution network data by pursuing a Bayesian approach. We present simulation results along with an application to Juventus Turin, Inter Milan, and other football clubs in the premier Italian soccer league.

==> summary_tables/crotone_formation_count.tex <==
\begin{table}[!htbp]
\centering
\caption{Number of passes and successful passes of Crotone during the 2020-2021 season,
by formation.}
\begin{tabular}{@{}lll@{}}
\toprule
Formation & Number of passes & Proportion of successful passes \\ \midrule
3-5-2          & 8125        & 84.53\% \\
5-3-2          & 3929        & 83.41\% \\
3-4-3          & 621         & 86.80\% \\
3-4-1-2        & 534         & 82.96\% \\
4-4-1          & 392         & 85.71\% \\
5-4-1          & 380         & 80.26\% \\
4-4-2          & 214         & 84.58\% \\
5-3-1          & 118         & 87.29\% \\
4-3-1-2        & 111         & 86.49\% \\
3-5-1          & 98          & 91.84\% \\
3-4-2-1        & 41          & 75.61\% \\
4-3-2          & 40          & 95.00\% \\
4-2-2-2        & 9           & 88.89\% \\ \bottomrule
\end{tabular}

\label{tab:formation_crotone}
\end{table}

==> summary_tables/fiorentina_formation_count.tex <==
\begin{table}[!htbp]
\centering
\caption{Number of passes and successful passes of Fiorentina during the 2020-2021 season,
by formation.}
\begin{tabular}{@{}lll@{}}
\toprule
Formation & Number of passes & Proportion of successful passes  \\ \midrule
3-5-2          & 8107        & 85.14\%  \\
5-3-2          & 1618        & 83.99\%  \\
4-4-2          & 1242        & 84.46\%  \\
3-4-3          & 1123        & 85.31\%  \\
4-3-1-2        & 496         & 84.27\%  \\
4-2-3-1        & 457         & 85.34\%  \\
4-1-4-1        & 410         & 81.46\%  \\
3-4-2-1        & 342         & 77.49\%  \\
3-5-1-1        & 299         & 81.94\%  \\
5-4-1          & 124         & 83.06\%  \\
3-5-1          & 93          & 86.02\%  \\
3-4-1-2        & 55          & 81.82\%  \\
4-3-1          & 32          & 68.75\%  \\
4-4-1          & 25          & 80.00\%  \\
4-3-2          & 18          & 61.11\%  \\
3-4-2          & 7           & 100.00\% \\ \bottomrule
\end{tabular}

\label{tab:formation_Fiorentina}
\end{table}

==> summary_tables/formation_observation_count.tex <==
\begin{table}[!htbp]
\centering
\caption{Number of passes during the 2020-2021 season,
by formation.}
\begin{tabular}{@{}ll}
\toprule
Formation & Number of observations \\ \midrule
3-5-2          & 71751                  \\
4-2-3-1        & 60868                  \\
4-4-2          & 31239                  \\
5-3-2          & 26442                  \\
4-3-3          & 24874                  \\
3-4-3          & 21912                  \\
3-4-2-1        & 19717                  \\
3-4-1-2        & 17454                  \\
4-1-4-1        & 12740                  \\
4-4-1-1        & 12568                  \\
4-3-1-2        & 10255                  \\
4-3-2-1        & 6786                   \\
3-5-1-1        & 3387                   \\
5-4-1          & 3368                   \\
4-4-1          & 2872                   \\
4-5-1          & 1814                   \\
4-1-3-2        & 1286                   \\
5-3-1          & 1018                   \\
4-3-2          & 770                    \\
3-4-2          & 219                    \\
4-1-3-1        & 207                    \\
3-5-1          & 195                    \\
3-2-3-2        & 73                     \\
4-3-1-1        & 64                     \\
4-3-1          & 32                     \\
4-2-1-2        & 12                     \\
4-2-1-3        & 12                     \\
4-2-2-2        & 9                      \\ \bottomrule
\end{tabular}

\label{tab:formation_rank}
\end{table}


==> summary_tables/genoa_formation_count.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{@{}lll@{}}
\toprule
Team Formation & Number of Passes & Successful Rate \\ \midrule
3-5-2         & 7061             & 83.64\%         \\
5-3-2         & 3726             & 83.17\%         \\
4-4-2         & 1450             & 82.55\%         \\
4-3-2-1       & 848              & 81.13\%         \\
4-3-1-2       & 683              & 79.36\%         \\
3-4-1-2       & 679              & 82.18\%         \\
5-4-1         & 223              & 88.79\%         \\
3-4-3         & 182              & 82.97\%         \\
3-4-2-1       & 123              & 87.80\%         \\
4-1-3-1       & 94               & 84.04\%         \\
3-5-1-1       & 90               & 90.00\%         \\
4-3-2         & 75               & 90.67\%         \\
4-3-3         & 75               & 85.33\%         \\
4-2-3-1       & 28               & 85.71\%         \\
4-3-1-1       & 5                & 20.00\%         \\ \bottomrule
\end{tabular}
\caption{Most Used Team Formation by Genoa}
\label{tab:formation_genoa}
\end{table}

==> summary_tables/positionPass.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{l|c}
Player Position                         & Successful Rate of Passes \\
\hline
Center Back                             & $91.71\%$                   \\
Right Center Back                       & $91.37\%$                 \\
Left Center Back                        & $91.23\%$                   \\
Left Defensive Midfielder               & $90.96\%$                   \\
Right Defensive Midfielder              & $89.72\%$                   \\
Right Center Back (3 at the back)       & $89.13\%$                   \\
Goalkeeper                              & $88.62\%$                   \\
Defensive Midfielder                    & $88.53\%$                   \\
Left Center Midfielder                  & $88.29\%$                   \\
Left Center Back (3 at the back)        & $88.04\%$                   \\
Right Center Midfielder                 & $87.95\%$                   \\
Left Center Midfielder (3 at the back)  & $84.09\%$                   \\
Right Back                              & $83.40\%$                   \\
Left Back                               & $82.69\%$                  \\
Attacking Midfielder                    & $82.51\%$                   \\
Right Center Midfielder (3 at the back) & $82.37\%$                   \\
Left Attacking Midfielder               & $81.67\%$                   \\
Left Wing Forward                       & $80.57\%$                   \\
Right Wing Forward                      & $80.29\%$                   \\
Left Wing                               & $80.11\%$                   \\
Right Attacking Midfielder              & $79.27\%$                   \\
Right Wing Back                         & $79.26\%$                   \\
Second Striker                          & $78.94\%$                   \\
Right Wing                              & $78.52\%$                   \\
Left Wing Back                          & $78.22\%$                   \\
Center Forward                          & $77.79\%$                   \\
Left Back (5 at the back)               & $77.19\%$                   \\
Right Back (5 at the back)              & $76.77\%$                  
\end{tabular}
\caption{Successful Rate of Passes of Each Position for the Whole Season}
    \label{tab:positionPass}
\end{table}

==> summary_tables/position_comp_3-5-2.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{@{}lll@{}}
\toprule
Position & Number of passes & Number of successful passes \\ \midrule
CB              & 8280             & 92.84\%         \\
RCB3            & 8593             & 90.36\%         \\
DMF             & 8935             & 89.04\%         \\
LCB3            & 8774             & 88.69\%         \\
GK              & 3772             & 87.99\%         \\
LCMF3           & 7086             & 84.18\%         \\
RCMF3           & 7128             & 83.02\%         \\
CF              & 3745             & 79.01\%         \\
SS              & 4049             & 78.74\%         \\
RWB             & 5761             & 78.48\%         \\
LWB             & 5594             & 77.48\%         \\ \bottomrule
\end{tabular}
\caption{
Team Formation 3-5-2: Comparison of Pass Accuracy by Positions}
\label{tab:352_accuracy_positions}
\end{table}

==> summary_tables/position_comp_4-4-2.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{@{}lll@{}}
\toprule
Player Position & Number of Passes & Successful Rate \\ \midrule
RCB              & 3417        & 91.81\% \\
LCB              & 3745        & 91.00\% \\
GK               & 1518        & 90.97\% \\
RCMF             & 3573        & 90.01\% \\
LCMF             & 3453        & 89.69\% \\
LB               & 3442        & 84.51\% \\
RB               & 3528        & 84.33\% \\
LW               & 2391        & 81.56\% \\
SS               & 1876        & 80.70\% \\
RW               & 2414        & 80.16\% \\
CF               & 1875        & 78.45\% \\ \bottomrule
\end{tabular}
\caption{Team Formation 4-4-2: Comparison of Pass Accuracy by Positions}
\label{tab:442_accuracy_positions}
\end{table}

==> summary_tables/teamPositionPass.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{l|l|c}
Team Name      & Player Position                        & Successful Rate of Passes \\
\hline
Atalanta       & Left Defensive Midfielder              & $93.86\%$                   \\
Benevento      & Left Defensive Midfielder              & $94.12\%$                   \\
Bologna        & Left Back (5 at the back)              & $96.00\%$                   \\
Cagliari       & Right Center Back                      & $89.47\%$                   \\
Crotone        & Left Defensive Midfielder              & $100.00\%$                  \\
       & Right Attacking Midfielder             & $100.00\%$                  \\
Fiorentina     & Right Defensive Midfielder             & $93.44\%$                   \\
Genoa          & Left Defensive Midfielder              & $100.00\%$                  \\
         & Right Defensive Midfielder             & $100.00\%$                  \\
Hellas Verona  & Defensive Midfielder                   & $94.74\%$                   \\
Internazionale & Left Center Back                       & $97.50\%$                  \\
Juventus       & Right Center Back                      & $94.62\%$                   \\
Lazio          & Left Defensive Midfielder              & $97.14\%$                   \\
Milan          & Left Back (5 at the back)              & $100.00\%$                  \\
        & Left Center Back (3 at the back)       & $100.00\%$                  \\
         & Left Center Midfielder (3 at the back) & $100.00\%$                  \\
        & Left Wing Forward                      & $100.00\%$                  \\
         & Right Center Back (3 at the back)      & $100.00\%$                  \\
        & Right Wing Forward                     & $100.00\%$                  \\
Napoli         & Center Back                            & $100.00\%$                  \\
       & Left Wing Back                         & $100.00\%$                  \\
       & Right Center Back (3 at the back)      & $100.00\%$                  \\
Parma          & Right Center Back                      & $91.44\%$                   \\
Roma           & Left Defensive Midfielder              & $94.32\%$                   \\
Sampdoria      & Defensive Midfielder                   & $93.40\%$                   \\
Sassuolo       & Right Center Back (3 at the back)      & $96.55\%$                   \\
Spezia         & Left Wing Back                         & $100.00\%$                  \\
        & Right Center Back (3 at the back)      & $100.00\%$                  \\
Torino         & Left Center Back                       & $93.51\%$                   \\
Udinese        & Right Defensive Midfielder             & $92.31\%$                  
\end{tabular}
\caption{Position(s) with Highest Successful Rate of Passes at Each Team for the Whole Season}
    \label{tab:teamPositionPass}
\end{table}

==> totalPass.tex <==
\begin{table}[!htbp]
    \centering
    \begin{tabular}{l|c c c}
          & \multicolumn{3}{c}{Successful proportion of passes}  \\
        Team & Total & First half & Second half \\
        \hline
Sassuolo& $89.47\%$ & $89.97\%$ & $88.92\%$ \\
Juventus&$88.95\%$ & $89.56\%$ & $88.27\%$ \\
Internazionale& $88.55\%$ & $88.69\%$ & $88.40\%$ \\
Napoli& $88.10\%$ & $88.67\%$ & $87.46\%$ \\
Roma& $86.44\%$ & $87.17\%$ & $85.65\%$ \\
Atalanta& $86.33\%$ & $86.33\%$ & $86.32\%$ \\
Milan & $86.22\%$ & $86.59\%$ & $85.82\%$ \\
Lazio & $85.91\%$ & $86.36\%$ & $85.43\%$ \\
Parma & $85.07\%$ & $85.86\%$ & $84.27\%$ \\
Udinese & $84.79\%$ & $85.57\%$ & $84.01\%$ \\
Torino & $84.68\%$ & $85.75\%$ & $83.53\%$ \\
Fiorentina & $84.50\%$ & $85.37\%$ & $83.64\%$ \\
Bologna & $84.45\%$ & $84.71\%$ & $84.17\%$ \\
Spezia & $84.39\%$ & $84.84\%$ & $83.91\%$ \\
Crotone & $84.28\%$ & $84.53\%$ & $84.01\%$ \\
Cagliari & $83.50\%$ & $84.41\%$ & $82.55\%$ \\
Genoa & $83.20\%$ & $84.13\%$ & $82.27\%$ \\
Benevento & $81.70\%$ & $81.52\%$ & $81.87\%$ \\
Hellas Verona & $81.39\%$ & $82.14\%$ & $80.58\%$ \\
Sampdoria & $81.35\%$ & $81.97\%$ & $80.70\%$ \\
    \end{tabular}
    \caption{Successful proportion of passes by teams during the 2020-2021 season of the Italian premier soccer league Serie A.}
    \label{tab:totalPass}
\end{table}

